Cinematographic Camera Diffusion Model

Designing effective camera trajectories in virtual 3D environments is a challenging task even for experienced animators. Despite an elaborate film grammar, forged through years of experience, that enables the specification of camera motions through cinematographic properties (framing, shots sizes, angles, motions), there are endless possibilities in deciding how to place and move cameras with characters. Dealing with these possibilities is part of the complexity of the problem. While numerous techniques have been proposed in the literature (optimization-based solving, encoding of empirical rules, learning from real examples,...), the results either lack variety or ease of control. In this paper, we propose a cinematographic camera diffusion model using a transformer-based architecture to handle temporality and exploit the stochasticity of diffusion models to generate diverse and qualitative trajectories conditioned by high-level textual descriptions. We extend the work by integrating keyframing constraints and the ability to blend naturally between motions using latent interpolation, in a way to augment the degree of control of the designers. We demonstrate the strengths of this text-to-camera motion approach through qualitative and quantitative experiments and gather feedback from professional artists. The code and data are available at \URL{https://github.com/jianghd1996/Camera-control}.

==> 4_feature_selection.tex <==


% \subsection{Feature extraction from broadcast clips}
% \XW{we should put this ahead of previous section}
% \VO{Our goal is to produce an edit that is not constrained to the camera positions and angles available to the current UFC broadcast~\XW{we need to say after statistic analysis}. To achieve our goal, we manually selected features that at present drive the choices of the UFC director during a fight. In particular, we chose four features: visibility, body orientation, body orientation~\XW{two orientations?}, distance between the fighters and their motion. These features are discussed in detail in the following subsections. }



% \VO{We used Dope + LCRNET (ref)~\XW{citation} to extract the poses of the fighters. Its output allows us to obtain 2D poses in the screen (image) space and a 3D estimated pose. When players are close together, and they are grappling, there are many obstructions and the extraction of the poses becomes more challenging. To disambiguate the players in close proximity, we also used the face detector provided by MovieNet (ref) to extract faces of the fighters. AND THEN?
% We separate the fight into two states: grappling state and non-grappling state. Grappling state corresponds to the game states where fighters are grappling each other and poses can't be well estimated. Non-grappling state includes game states where there is some distance between the players andit is possible to use the poses to evaluate the features.}

%As our goal is to produce an edit that can be done with camera positions and angles never seen in UFC broadcast, we decided to manually select the features that drives the choices of the editor during the fight. We select four features that are rather common in editing: visibility, body orientation, distance between fighters and joint motion. Each of them would be discuss in more detail later on.

%We used Dope + LCRNET (ref) to extract the poses of the fighters as it allow us to obtain 2d poses in screen space and a 3d estimated pose.

%Due to the difficulty of obtaining poses when fighters are grappling each other, we also used the face detector provided by MovieNet (ref) to extract faces of the fighters. We will separate the fight into two state: grappling state and non-grappling state. Grappling state correspond to the frames where the fighters are grappling each other and the poses can't be well estimated. Non-grappling state is the other state in which we can use the poses to evaluate the features.

%In this paper, we denote \( C \) the set of all cameras, \(P\) the set of fighters, \(J\) the set of joint for a pose, \(I\) the set of all frames and \( I^{c}_{p} \subset I\), \(c \in C\), \(p \in P\) as the set of frames on which the pose of the fighter \(p\) has been detected on the camera \(c\).

%For all \(c \in C\), \( p \in P\), \(i \in I^{c}_{i}\), \(j \in J\):

%\( x^{c}_{p,i,j} \in \mathbb{R}^{3}\) represent the position of the joint \(j\) of fighter \(p\) at frame \(i\) of camera \(c\) in the 3d pose referential.

%\(\hat{x}^{c}_{p,i,j} \in \mathbb{R}^{2}\) the position of the fighter \(p\) \(j\) joint at frame \(i\) on the camera \(c\) screen, in pixel. 



\subsection{Feature selection}

%Evaluating the impact on those features in the edit means determining if there are relevant or not for choosing a camera rather than another. To do this we perform a t-test to evaluate if the mean of the feature on the frame used during broadcast is greater or less than the mean on the ones that are not used. The variance of the scores in each group are likely to not be equal so to perform this test we are going to use a one-tailored Welch's t-test.

%To get more information about the importance of the feature we calculate the Pearson correlation coefficient between the array of scores for each frame and an array of 1 if the frame is used in broadcast and 0 otherwise. The Pearson coefficient allow us to know how much the choice of the camera is linear to the score. A score of absolute value close to 1 indicate a strong linear correlation and so that the feature is a good feature. One close to 0 indicate that the feature is irrelevant. A positive (resp negative) coefficient indicate that a high (resp low) score induce a choice of the frame.

\VO{We evaluate the impact of these features on the camera selection performing a t-test, checking for each feature \dots }

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.5]{Figure/VisibilityBodyOrientPearsonLive2.png}
%     \caption{Visibility and Body Orientation score Pearson coefficient in function of the window size used for the weighted moving average}
%     \label{fig:MAScore}
% \end{figure}

% Extracting good visualisation feature is hard process. Each cameraman is always trying to film the best way possible and so the choice to select a camera rather than another will consist of choosing one camera in a set of camera that can also be very good candidate. If we look at the distribution of the score onto the selected frame and the one not selected, it is likely that the difference between the two will be small because the set of unused camera can contained camera that aren't bad compared to the chosen one.

% To evaluate the different feature, we do a multiple step process. First we will look at the distribution of the feature's score over the set of frame chosen during broadcast and the ones that are not. It is very likely that even for a good feature the distribution will not show great distinction as the cameramen are always trying to maximise them. Secondly, because the edit consist of choosing one camera over a set of multiple camera that can also have very good score, we look at the probability of a camera being chosen knowing that it has the best score on a frame.
% Thirdly, it is rather obvious that an editor will not chose a camera that has been very good only on one frame. To take into account the time context we will perform a weighting moving average on the score of each camera with different window size. The weights of the moving average will correspond to a truncated Gaussian weighting taking into account only the scores previous to the current frame as to perform a calculation in 'live'.

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.3]{Figure/VisuDistri.png}
%     \caption{Visibility Score Distribution}
%     \label{fig:VisScore}
% \end{figure}

% The distribution of the visibility score can be seen on figure \ref{fig:VisScore}. We see that the chosen camera seem to have more frame with good visibility but the difference is not large enough to make a decision.
% The probability of the camera being chosen while having the best score is around 0.22, close to 1/5. This indicate us that is not good enough to choose the good camera from the set of 5 camera.
% Taking into account the time context we can observe on figure \ref{fig:VisWin} that applying our weighted moving average with a window size off 200 can make the probability go has up as 0.42 meaning that the camera with the best has 1/2 chance to be the one selected. The rise of the probability can be explained by the fact that a camera which has a better visibility during the last 200 frames is more likely to be chosen. The decrease of the probability after 200 show that if we take into account too much knowledge of the past we loose information on the current frame.

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.3]{Figure/VisuProbaWin.png}
%     \caption{Camera Probability to be chosen knowing that it has the maximum visibility score}
%     \label{fig:VisWin}
% \end{figure}

% Visibility is a necessary criterion to explore further features. Because we can't estimate some of the features when the fighters are not visible. We have to select it has one of the features.

% The distribution of the orientation score when the two player are visible (figure \ref{fig:OrientDistri}) show us that the camera are mostly filming them with a score of around 0.5. Because the player are mostly looking at them, there is not a lot of frame with the two fighter oriented toward the camera at the same time. The probability of the best camera being is chosen based on this score when the two fighter are visible is around 0.25 which do not indicate a strong correlation.

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.3]{Figure/orientDistrivP1P2.png}
%     \caption{Orientation Score Distribution}
%     \label{fig:OrientDistri}
% \end{figure}



% Plot Distri new Score

% We observe on figure \ref{fig:OrientWin} that a window size between 300 and 700 frames gives a better probability for the camera with the best score to be the one chosen. With a window size of 300, the probability is around 0.46.

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.3]{Figure/OrientWindoScore.png}
%     \caption{Camera Probability to be chosen knowing that it has the maximum score}
%     \label{fig:OrientWin}
% \end{figure}

% Looking at the distance distribution between the fighter, we see that for the frame used during broadcast the distance follow a uniform distribution between 0.2 and 1.3 pixel/width ratio. We conclude that the distance is not relevant when selecting the camera. However we can clearly see that a lot of frame that are not being chosen have a small distance between the fighters. We interpret this result as a correlation between the small distance and both the players and the camera being aligned. In such configuration, the camera is not chosen because the fighters are not well oriented toward the camera and not because they have a small distance between them.

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.3]{Figure/DistBtPlayerDistri.png}
%     \caption{Camera Probability to be chosen knowing that it has the maximum score}
%     \label{fig:DistDistri}
% \end{figure}









==> 5_results_backup.tex <==







% \begin{figure}[ht]
%     \centering
%     \includegraphics[clip,width=0.47\textwidth]{Figure/interpolating.pgf}{\centering}
%     \caption{Visualization of keyframe constrained CLIP interpolated results between rotation (blue) and pan (purple).}
%     \label{fig:viz_traj_interpolation}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[clip,width=0.47\textwidth]{Figure/interpolating.pgf}{\centering}
%     \caption{Visualization of keyframe constrained CLIP interpolated results between rotation (blue) and pan (purple).}
%     \label{fig:viz_traj_interpolation}
% \end{figure}

% \begin{table*}[h!]
%     \centering
%     \begin{tabular}{l|c|c|c}
%         \hline
%             Method & FID$\downarrow$ & Keyframe distance $\downarrow$ & classification accuracy $\uparrow$  \\
%         \hline
%          LSTM+CLIP(1-to-1) & 1.44 & 0.14 & 88.8 \\
%          LSTM+CLIP(1-to-N) & 1.24 & 0.17 & 88.76 \\
%          LSTM+CLIP+$\mathcal{L}_K$(1-to-1) & 0.34 & 0.046 & 93.8 \\
%          LSTM+CLIP+$\mathcal{L}_K$(1-to-N) & 0.17 & 0.036 & 96.98  \\
%         \hline
%          Ours (inpainting) & 0.75 & 0.47 & 94.2 \\
%          Ours (inpainting+noise) & 1.91 & 0.92 & 79.2 \\
%          Ours(w=0.5) & 0.068 & 0.037 & 98.5 \\
%          Ours(w=1) & 0.059 & 0.039 & 98.4 \\
%          Ours(w=2) & 0.29 & 0.077 & 95.2 \\
%          Ours (no style) & 0.14 & 0.051 & 97.3 \\
%         \hline
%     \end{tabular}
%     \caption{We evaluate the FID and shot classification accuracy on with gt test keyframe.}
%     \label{tab:keyframe}
% \end{table*}

% \begin{table*}[h!]
%     \centering
%     \begin{tabular}{l|c|c|c}
%         \hline
%             Method & FID$\downarrow$ & Keyframe distance $\downarrow$ & classification accuracy $\uparrow$  \\
%         \hline
%          LSTM+CLIP(1-to-1) & 2.57 & 0.125 & 48.21 \\
%          LSTM+CLIP(1-to-N) & 2.16 & 0.112 & 48.53 \\
%          LSTM+CLIP+$\mathcal{L}_K$(1-to-1) & 1.81 & 0.050 & 47.98 \\
%          LSTM+CLIP+$\mathcal{L}_K$(1-to-N) & 1.79 & 0.039 & 46.51  \\
%         \hline
%          Ours (inpainting) & 2.69 & 0.556 & 68.65 \\
%          Ours (inpainting+noise) & 2.21 & 0.706 & 70.27 \\
%          Ours(w=0.5) & 1.92 & 0.037 & 49.28 \\
%          Ours(w=1) & 1.89 & 0.040 & 49.04 \\
%          Ours(w=2) & 1.72 & 0.079 & 47.06 \\
%          Ours (no style) & 1.89 & 0.054 & 48.25 \\
%         \hline
%     \end{tabular}
%     \caption{We evaluate the FID and shot classification accuracy with random test keyframe.}
%     \label{tab:keyframe_rand}
% \end{table*}

% \begin{table*}[h!]
%     \centering
%     \begin{tabular}{l|c|c|c}
%         \hline
%             Method & FID$\downarrow$ & Keyframe distance $\downarrow$ & classification accuracy $\uparrow$  \\
%         \hline
%          LSTM+CLIP(1-to-1) & 15.55 & 0.667 & 23.97 \\
%          LSTM+CLIP(1-to-N) & 14.12 & 0.716 & 23.97 \\
%          LSTM+CLIP+$\mathcal{L}_K$(1-to-1) & 16.11 & 0.383 & 23.80 \\
%          LSTM+CLIP+$\mathcal{L}_K$(1-to-N) & 16.09 & 0.343 & 24.36 \\
%         \hline
%          Ours (inpainting) & 15.36 & 1.824 & 41.63 \\
%          Ours (inpainting+noise) & 14.38 & 2.096 & 44.4 \\
%          Ours(w=0.5) & 15.58 & 0.363 & 24.80 \\
%          Ours(w=1) & 15.68 & 0.374 & 24.68 \\
%          Ours(w=2) & 15.80 & 0.375 & 24.56 \\
%          Ours (no style) & 15.50 & 0.324 & 24.88 \\
%         \hline
%     \end{tabular}
%     \caption{We evaluate the FID and shot classification accuracy with random test keyframe from whole dataset.}
%     \label{tab:keyframe_randA}
% \end{table*}

% method :
% 1. keyframe based + example paper
% 2. inpainting
% 3. keyframe condition generation
% metric :
% 1. keyframe distance
% 2. continuity
% 3. style classifier




% More Moving camera within prompt

% Transition better than blender

% Text, video mixed (real be more interesting)

% At which point the camera should change 

% Keyframes + variations

% Switch between multiple characters, CUT / smooth transition ? 

% Long scripts -> ChatGPT -> formatted scripts. Make the low level control reliable. Leave the high level to LLM.

% Smooth character trajectories.


% \begin{table*}[h!]
%     \centering
%     \caption{We evaluate the FID and shot classification accuracy on with gt test keyframe and arbitrary test keyframe.}
%     \begin{tabular}{l|c|c|c|c|c|c}
%         \hline
%             & \multicolumn{3}{|c|}{Test with gt keyframe} & \multicolumn{3}{|c}{Test with arbitrary keyframe}\\
%         \hline
%             Method & FID$\downarrow$ & Keyframe distance $\downarrow$ & R Precision $\uparrow$ & FID$\downarrow$ & Keyframe distance $\downarrow$ & R Precision $\uparrow$\\
%         \hline
%          LSTM+CLIP(1-to-1) & 1.44 & 0.14 & 88.8 & 2.57 & 0.125 & 48.21\\
%          LSTM+CLIP(1-to-N) & 1.24 & 0.17 & 88.76 & 2.16 & 0.112 & 48.53 \\
%          % LSTM+CLIP+$\mathcal{L}_K$(1-to-1) & 0.34 & 0.046 & 93.8 & 1.81 & 0.050 & 47.98\\
%          % LSTM+CLIP+$\mathcal{L}_K$(1-to-N) & 0.17 & 0.036 & 96.98 & 1.79 & 0.039 & 46.51  \\
%         \hline
%          Ours (inpainting) & 0.75 & 0.47 & 94.2 & 2.69 & 0.556 & 68.65 \\
%          % Ours (inpainting+noise) & 1.91 & 0.92 & 79.2 & 2.21 & 0.706 & 70.27 \\
%          % Ours(w=0.5) & 0.068 & 0.037 & 98.5 & 1.92 & 0.037 & 49.28  \\
%          Ours(w=1) & 0.059 & 0.039 & 98.4 & 1.89 & 0.040 & 49.04 \\
%          % Ours(w=2) & 0.29 & 0.077 & 95.2 & 1.72 & 0.079 & 47.06 \\
%          % Ours (no style) & 0.14 & 0.051 & 97.3 & 1.89 & 0.054 & 48.25 \\
%         \hline
%     \end{tabular}
%     \label{tab:keyframe}
% \end{table*}



==> 6_limitations.tex <==


\subsection{formatted language VS natural language}


\paragraph{User Study}

\paragraph{Engage with ChatGPT}

% \paragraph{Obstacle avoidance}

==> 8_all_image_page.tex <==

% \newpage
% \begin{figure*}[ht]
%     \centering
%     \includegraphics[clip,width=.9\textwidth]{Figure/allImage_page2.png}{\centering}
%     \caption{We provide demonstrations of i) demo of transition scheme, which involves linear interpolation on CLIP text embeddings between different styles while adhering to keyframing constraints. For instance, we showcase transitions between rotation and pan movements, with each step a 20\% increment in the interpolation. The generated results maintains the desired style, and satisfy the specified keyframe conditions with smoothness; ii) examples of casual language input, showing that our method can handle non-strict cinematographic language to a certain extent, though erroneous results can still occur in some cases; iii) comparison of different transition schemes, our proposed transition can smoothly connect different styles with no need of transition script.}
%     \label{fig:all_image_page2}
% \end{figure*}
